Why are optical coronal lines faint in active galactic nuclei?

Forbidden collisionally excited optical atomic transitions from high ionization potential (IP$\geq$54.8\,eV) ions, such as Ca$^{\mathrm{4+}}$, Ne$^{\mathrm{4+}}$, Fe$^{\mathrm{6+}}$, Fe$^{\mathrm{10+}}$, Fe$^{\mathrm{13+}}$, Ar$^{\mathrm{9+}}$, and S$^{\mathrm{11+}}$, are known as optical coronal lines (CLs). The spectral energy distribution (SED) of active galactic nuclei (AGN) typically extends to hundreds of electron volts and above, which should be able to produce such highly ionized gas. However, optical CLs are often not detected in AGN. Here we use photoionization calculations with the \textsc{Cloudy} spectral synthesis code to determine possible reasons for the rarity of these optical CLs. We calculate CL luminosities and equivalent widths from radiation pressure confined photoionized gas slabs exposed to an AGN continuum. We consider the role of dust, metallicity, and ionizing SED in the formation of optical CLs. We find that (1) dust reduces the strength of most CLs by $\sim$three orders of magnitude, primarily as a result of depletion of metals onto the dust grains. (2) In contrast to the CLs, the more widely observed lower IP optical lines such as [O\, III] 5007\,\AA, are less affected by depletion and some are actually enhanced in dusty gas. (3) In dustless gas many optical CLs become detectable, and are particularly strong for a hard ionizing SED. This implies that prominent CL emission likely originate in dustless gas. Our calculations also suggest optical CL emission is enhanced in galaxies with low mass black holes characterized by a harder radiation field and a low dust to metal ratio. The fact that optical CLs are not widely observed in the early universe with JWST may point to rapid dust formation at high redshift.

==> line_table.tex <==
\begin{table*}\label{linetable}
\caption{Table of 12 optical CLs to be considered in this study along with their critical densities, IPs, and transitions.}
\begin{tabular}{lcccc}
\hline
\hline
Line          & Wavelength (\AA)$^1$ & Critical Density (cm$^{-3}$) & Ionization Potential (eV)$^{2}$ & Transition                                                                             \\ \hline
{[}Fe\,V{]}   & 3891.28                         & $1.61\times 10^{8}$          & 54.84                     & $^{5}$D$_{4}-^{3}$F$2_{4}$                                                        \\
{[}Ca\,V{]}   & 5309.11                         & $6.36\times 10^{7}$          & 67.10                     & $^{3}$P$_{2}-^{1}$D$_{2}$                                                \\
{[}Fe\,VI{]}  & 5335.18                         & $6.32\times 10^{6}$          & 75.00                     & $^{4}$F$_{3/2}-^{4}$F$_{1/2}$                                            \\
{[}Fe\,VI{]}  & 5176.04                         & $3.29\times 10^{7}$          & 
75.00                     & $^{4}$F$_{9/2}-^{2}$G$_{9/2}$
\\
{[}Ne\,V{]}   & 3425.88                         & $1.90\times 10^{7}$          & 97.11                     & $^{2}$P$_{2}-^{1}$D$_{2}$                                                \\
{[}Fe\,VII{]} & 6087.00                         & $4.46\times 10^{7}$          & 99.00                     & $^{3}$F$_{3}-^{1}$D$_{2}$                                                              \\
{[}Fe\,VII{]} & 4893.37                         & $3.09\times 10^{6}$          & 99.00                     & $^{3}$F$_{2}-^{3}$P$_{1}$                                                              \\
{[}Fe\,X{]}   & 6374.51                         & $4.45\times 10^{8}$          & 235.04                    & $^{2}$P$_{3/2}^{0}-^{2}$P$_{1/2}^{0}$                                                  \\
{[}Fe\,XI{]}  & 7891.80                         & $6.39\times 10^{8}$          & 262.10                    & $^{3}$P$_{2}-^{3}$P$_{1}$                                                              \\
{[}Fe\,XIV{]} & 5302.86                         & $3.99\times 10^{8}$          & 361.00                    & $^{2}$P$_{1/2}^{0}-^{2}$P$_{3/2}^{0}$                                                  \\
{[}Ar\,X{]}   & 5335.27                         & $2.36\times 10^{9}$          & 422.60                    & $^{2}$P$_{3/2}^{0}-^{2}$P$_{1/2}^{0}$                                                  \\
{[}S\,XII{]}  & 7611.00                         & $7.09\times 10^{9}$          & 504.78                    & $^{2}$P$_{1/2}^{0}-^{2}$P$_{3/2}^{0}$                                                  \\ \hline
\end{tabular}
\begin{tablenotes}
	\item[0] \textsuperscript{1}Wavelengths taken from: \url{https://physics.nist.gov/PhysRefData/ASD/lines_form.html}.
	\item[1] \textsuperscript{2}Ionization potential taken from: \url{https://physics.nist.gov/PhysRefData/ASD/ionEnergy.html}.
\end{tablenotes}
\end{table*}
